Navigating the Minefield of MT Beam Search in Cascaded Streaming Speech Translation

We adapt the well-known beam-search algorithm for machine translation to operate in a cascaded real-time speech translation system. This proved to be more complex than initially anticipated, due to four key challenges: (1) real-time processing of intermediate and final transcriptions with incomplete words from ASR, (2) emitting intermediate and final translations with minimal user perceived latency, (3) handling beam search hypotheses that have unequal length and different model state, and (4) handling sentence boundaries. Previous work in the field of simultaneous machine translation only implemented greedy decoding. We present a beam-search realization that handles all of the above, providing guidance through the minefield of challenges. Our approach increases the BLEU score by 1 point compared to greedy search, reduces the CPU time by up to 40% and character flicker rate by 20+% compared to a baseline heuristic that just retranslates input repeatedly.

==> modified_v1.tex <==
\section{Introduction}

The field of live speech translation has seen significant advancements in recent years, particularly in the area of real-time simultaneous text-to-text machine translation. 
In contrast, our research concentrates on the real-time decoding aspect, with a specific emphasis on the beam search aspect.
The cascaded live speech translation system we propose is composed of several components - automatic speech recognition (ASR), machine translation (MT), text-to-speech (TTS) or display. The data flow is as follows: ASR receives a live audio stream from the microphone and generates a stream of transcription events which may be \textit{intermediate} or \textit{final}. 


MT processes the stream of transcription events and generates a corresponding stream of translation events (\textit{intermediate} or \textit{final}) which are either sent to the display or to TTS which generates an audio stream that is played to the loudspeaker. The MT component must be able to correctly process both intermediate and final events and propagate them to the output.

\begin{figure}[h]
\centering
% \includegraphics[width=0.5\textwidth]{figure.png}
\caption{[TODO: Insert figure here]}
\label{fig:todo}
\end{figure}


To understand our algorithm and its complexity, we introduce the core concept of {\em intermediate} and {\em final} events that flow through the system. \emph{Intermediate} events denote a speech-recognition result that is not stable, while \emph{Final} events denote speech-recognition results that won't change anymore. A key goal of our streaming beam search for MT is that, like ASR, it too generates intermediate and final outputs. These intermediate and final outputs are processed by display and TTS. Display shows both intermediate and final outputs, while TTS can only pronounce finals because it cannot go back on what it already said.
While previous works have implemented greedy decoding, our research introduces the implementation of beam search decoding. Furthermore, we have integrated this beam search decoder into a pipeline that transcribes audio in real-time, displaying translations in real-time or playing translations through a text-to-speech system (TTS). This integration introduces an additional layer of complexity to the beam search algorithm.

Our approach is compared with a method that simulates streaming using a non-streaming model. This method serves as a useful baseline for display output but is unsuitable for TTS output due to its high user-perceived latency and computational inefficiency.

Our research has yielded the following results:
\begin{itemize}
\item
  An increase in BLEU score by 1 point compared to greedy for a beam size of 3.
\item
  A reduction of almost 40\% in CPU time compared to fake streaming with repeated retranslations, depending on the beam size on ASR data.
\item
  A 21\% decrease in character flicker compared to fake streaming with repeated retranslations.
\item
  An improvement in the BLEU score by 0.6 compared to streaming greedy decoding from the Seamless SimulEval library through our implementation of streaming greedy decoding.
\end{itemize}


\section{Background}
\hypertarget{fake-streaming-baseline}{%
\subsection{Faking Streaming by Repeated Retranslation}\label{fake-streaming-baseline}}

% [Frank: Can't we just ``fake'' streaming translation by repeated retranslation?]
The baseline approach utilizes a traditional encoder-decoder MT model that accepts a complete sentence as input and translates it into another language. This non-streaming model can be adapted to simulate streaming by retranslating the entire input received so far for the current sentence each time an additional event arrives at MT. However, this repeated retranslation is computationally inefficient ($O(T^2)$) due to the redundancy of computations. Furthermore, this approach is incompatible with Text-to-Speech (TTS) output, as partial translations cannot be overwritten. To overcome these limitations, a streaming MT model is proposed. This model maintains a state and, upon receiving a new transcription, processes it and decides whether to read more tokens or emit tokens to the output. The emitted tokens are considered final and cannot be altered. The streaming MT model addresses two key issues: it reduces computational cost when translating to display and minimizes latency from whole-sentence to a few words when translating to audio.


\hypertarget{model-architecture}{%
\subsection{Streaming Model Architecture}\label{model-architecture}}

The MT model comprises two components -- the encoder and the decoder, both of which employ a Transformer architecture \cite{VaswaniSPUJGKP17}. The streaming-MT decoder model not only returns a probability distribution over tokens at each timestamp but also a "write" probability. If the "write" probability falls below a certain threshold, it indicates that the model has not ingested sufficient input to generate the next token. Consequently, another input token is ingested instead of generating a token for output.
The model is trained with dual objectives: to maximize the log probability of a sequence and to minimize expected latency. The module that computes expected latency utilizes the "write" probability. Over time, several methods have been developed to compute the encoder-decoder cross-attention. The current state-of-the-art approach is Monotonic Infinite Lookback (MILK) \cite{milk}, which also prescribes how the "write" probability is computed.
Let $P$ be the probability distribution over tokens, $W$ be the "write" probability, and $T$ be the threshold. If $W < T$, another input token is ingested:
\begin{equation}
\text{Ingest another input token} =
\begin{cases}
\text{True,} & \text{if } W < T \
\text{False,} & \text{otherwise}
\end{cases}
\end{equation}
The model is trained to maximize the log probability of a sequence $L$ and minimize expected latency $E$:
\begin{equation}
\text{Maximize } L \text{ and minimize } E
\end{equation}












\hypertarget{non-streaming-beam-search-baseline}{%
\subsection{Baseline: Non-streaming Beam Search}\label{non-streaming-beam-search-baseline}}
The non-streaming beam search is a well-established and relatively
uncomplicated method. The term ``beam'' denotes the collection of the
highest-scoring $k$ hypotheses during the incremental decoding process. In
the non-streaming context, the encoder is initially run on the entire
sequence. Subsequently, a single step of the decoder is executed for each of
the (up to) $k$ hypotheses in the current beam in a loop. This expands each
hypothesis by all $n$ words in the vocabulary, resulting in up to $n \cdot k$
expanded hypotheses, which are then sorted according to their score. The top $k$ are iterated
through, setting aside those that are complete (terminated with
\verb+<EOS>+ or exceeded the maximum length). The first $k$ incomplete hypotheses are then selected and the expansion of these hypotheses continues until $k$ complete hypotheses are obtained. The top hypothesis is then returned.


\section{Streaming-MT Beam Search}
In the streaming context, the model decides whether to write a new input token or read and encode another one. This is facilitated by an additional component in the MT model that calculates a ``write'' probability. The challenge of each hypothesis in the beam potentially having read and written a different number of tokens is addressed by maintaining a set of hypotheses that have read the same number of tokens from the input. Hypotheses that decided to write are continuously expanded until only those that want to read remain. 
During expansion, hypotheses are scored and the top $k$ selected. 
Once all top $k$ hypotheses want to read, a read is performed for all. 
The write expansion loop is then resumed and continues until all tokens have been read (reached \verb+<EOS>+). 
This ensures that at any given time, all hypotheses in the beam have read the same input tokens.

\subsection{RNN-T Beam Search}
For comparison, a similar decoding algorithm is used for an ASR model known as RNN-T. The RNN-T model also generates a ``read'' probability, expressed in the form of the ``blank'' token. The RNN-T beam search maintains two sets of hypotheses: $A$ - the set of hypotheses that have read n tokens and $B$ - the set of hypotheses that have read n + 1 tokens. In every iteration, the hypothesis with the best score is removed from set $A$, expanded, and then all tokens are looped over. For each token, a new hypothesis is created and inserted into set $A$. Any hypothesis expanded with the blank token (indicating ``read``), is pushed into set $B$ because the blank token essentially means to read a new token.

\subsection{State Management}

Given that ASR inputs arrive in real time, a ``read'' decision may refer to an input token that has not yet been spoken or recognized, necessitating the decoder to yield the CPU until the next ASR event. This implies that the internal decoding state must be carried across incremental invocations of the decoder. Specifically, the list of the current hypotheses must be maintained, and for each hypothesis, the encoder and decoder model state, along with a few other variables, need to be stored. This will be referred to as the beam search state.

Let $H$ be the set of current hypotheses, $E$ be the encoder state, $D$ be the decoder state, and $V$ be the set of other variables. The beam search state $S$ is then defined as:

\begin{equation}
S = \{H, E, D, V\}
\end{equation}

\subsection{Emitting Output}

The goal is to write intermediate outputs to the display while decoding the input to enhance user-perceived latency. There are two types of outputs -- intermediate and final. A final output is a prefix of the output that will remain unchanged -- it will not be rewritten. An intermediate output can change, so the user might experience a slight flicker when words are overwritten on the display.

Let $O$ be the output, $F$ be the final output, and $I$ be the intermediate output. If $O$ is a prefix of the final output, it is considered as $F$ and will not be rewritten. Otherwise, $O$ is considered as $I$ and can be changed.

\begin{equation}
O = 
\begin{cases} 
F, & \text{if } O \text{ is a prefix of the final output} \\
I, & \text{otherwise}
\end{cases}
\end{equation}



\subsection{Handling Incomplete Words from ASR}
ASR can return incomplete word prefixes in the stream of inputs. For instance, the word ``\_carpet'' might be recognized as two tokens ``\_car'' followed by ``pet``, and these may be emitted in two consecutive final events. The challenge with incomplete words is that the tokenization of the word can alter once the rest of the word is received -- while the ASR vocabulary may not have a whole-word entry for ``\_carpet``, the MT vocabulary may. This is addressed by treating the prefix that terminates at a word boundary (space or punctuation) as finalized input. The remainder of the input string, whose stable tokenization cannot be determined, is treated as intermediate input.
Let $W$ be a word, $P$ be a prefix of $W$ that ends at a word boundary, and $R$ be the remainder of the input string. If $P$ is recognized as a whole-word entry in the MT vocabulary, it is treated as finalized input. Otherwise, $R$ is treated as intermediate input.
\begin{equation}
P =
\begin{cases}
\text{finalized input,} & \text{if } P \text{ is recognized as a word} \\
\text{intermediate input,} & \text{otherwise}
\end{cases}
\end{equation}


\subsection{Scoring Beams}
In order to rank beams, a score for each beam must be computed. The optimal method for score computation in the case of a streaming NMT model is not entirely clear. We experimented with incorporating the heuristic read/write probability into the path score of a beam, but this approach was not successful. The method that we ultimately adopted was that the score of a beam is the length-normalized token sequence probability, excluding the read/write probability entirely.
Let $B$ be a beam, $L$ be the length of the token sequence in $B$, and $P$ be the token sequence probability. The score $S$ of $B$ is computed as:
\begin{equation}
S(B) = \frac{P}{L}
\end{equation}


\subsection{Batching}
Batching multiple model evaluations can significantly improve inference time, as model inference is more influenced by memory bandwidth than compute cycles. While batching is straightforward in non-streaming beam search due to equal length hypotheses, it's more complex in the streaming case due to differing token sequences for each beam. This issue could be mitigated with an LSTM decoder, but this may compromise accuracy. Despite these challenges, batching is beneficial as it allows for the same encoder state to be held for all beams, which read simultaneously.
Let $N$ be the number of beams, $D$ be the decoder weight, and $T$ be the time taken for one decoding step. Without batching, the time taken is:
\begin{equation}
T = N \times D
\end{equation}
With batching, the time taken is:
\begin{equation}
T = D
\end{equation}
Our experiments demonstrated that batching beams significantly accelerates the performance of one decoding step. This is because we only need to transfer decoder weight from DRAM to CPU cache once. Without batching, we need to copy the weights once for each beam, so the speed deteriorates drastically with the number of beams.
